GAF: Gaussian Avatar Reconstruction from Monocular Videos via Multi-view Diffusion

We propose a novel approach for reconstructing animatable 3D Gaussian avatars from monocular videos captured by commodity devices like smartphones. Photorealistic 3D head avatar reconstruction from such recordings is challenging due to limited observations, which leaves unobserved regions under-constrained and can lead to artifacts in novel views. To address this problem, we introduce a multi-view head diffusion model, leveraging its priors to fill in missing regions and ensure view consistency in Gaussian splatting renderings. To enable precise viewpoint control, we use normal maps rendered from FLAME-based head reconstruction, which provides pixel-aligned inductive biases. We also condition the diffusion model on VAE features extracted from the input image to preserve facial identity and appearance details. For Gaussian avatar reconstruction, we distill multi-view diffusion priors by using iteratively denoised images as pseudo-ground truths, effectively mitigating over-saturation issues. To further improve photorealism, we apply latent upsampling priors to refine the denoised latent before decoding it into an image. We evaluate our method on the NeRSemble dataset, showing that GAF outperforms previous state-of-the-art methods in novel view synthesis. Furthermore, we demonstrate higher-fidelity avatar reconstructions from monocular videos captured on commodity devices.

==> header.tex <==

\usepackage{booktabs} % For formal tables
\usepackage[ruled]{algorithm2e} % For algorithms
\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}

\usepackage{amsmath}
% \usepackage{amssymb}
\usepackage{subcaption}
\usepackage{tkz-euclide}
\usepackage{tikz}
% \usetkzobj{all}
\usepackage{pgfplots}
% \pgfplotsset{compat=1.14}
% \usetikzlibrary{positioning,calc,fadings,backgrounds,fit,3d,shapes.misc,shapes.geometric}
% \usetikzlibrary{matrix}

\usepackage{multirow}
% \usepackage{afterpage}

\usepackage{overpic}
\usepackage{color, colortbl}
\usepackage{xcolor}
% \definecolor{sim}{RGB}{246, 182, 13}
% \definecolor{interp}{RGB}{109, 212, 126}
% \definecolor{sim}{RGB}{0, 0, 0}
% \definecolor{interp}{RGB}{0, 0, 0}
% \definecolor{sim}{RGB}{244, 113, 116}
% \definecolor{interp}{RGB}{1, 121, 111}
\definecolor{sim}{RGB}{128,0,128}
% \definecolor{interp}{RGB}{0, 255, 0}
\definecolor{interp}{RGB}{255, 169, 0}

% Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% \makeatletter
% \DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

% \def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
% \def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
% \def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
% \def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
% \def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
% \def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
% \def\etal{\emph{et al}\onedot}
% \makeatother

\definecolor{mytbcol}{RGB}{175,227,246}
\newcommand{\MATTHIAS}[1]{{\bfseries \small \color{blue} Matthias: #1}}
\newcommand{\TODO}[1]{{ \small \color{red} TODO: #1}}
\newcommand{\jiapeng}[1]{{\bfseries \small \color{orange} Jiapeng: #1}}
\newcommand{\davide}[1]{{\bfseries \small \color{ForestGreen} Davide: #1}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator{\LPIPS}{LPIPS}
% \DeclareMathOperator{\PSNR{PSNR}
% \DeclareMathOperator{\SSIM}{SSIM}
\DeclareMathOperator{\rec}{rec}
\DeclareMathOperator{\view}{view}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\tgt}{tgt}
\DeclareMathOperator{\expr}{expr}
\DeclareMathOperator{\img}{img}
\DeclareMathOperator{\sds}{sds}
\DeclareMathOperator{\pos}{pos}
\DeclareMathOperator{\scale}{scale}
\DeclareMathOperator{\ssim}{ssim}
\DeclareMathOperator{\lpips}{lpips}
\DeclareMathOperator{\LPIPS}{LPIPS}
\DeclareMathOperator{\SSIM}{SSIM}

\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\expnumber}[2]{{#1}\mathrm{e}{#2}}
\renewcommand{\paragraph}[1]{\smallskip\noindent\textbf{#1}}

\usepackage{threeparttable}
% \usepackage{libertine}
% \usepackage{libertinust1math}
% \usepackage[T1]{fontenc}

==> tabs/ablation_306.tex <==
\begin{table}[t]%[!htbp]
        \vspace{-1mm}
	\renewcommand\arraystretch{1.2}
        \setlength{\tabcolsep}{2pt}
	\begin{center}
        \footnotesize
		\begin{tabular}{*{7}{c}}
                \toprule
                \multirow{2}*{Method} & \multicolumn{3}{c}{Novel-View Synthesis}   & \multicolumn{3}{c}{Self-Reenactment}  \\
			\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
                     & LPIPS $\downarrow$  & PSNR $\uparrow$ & SSIM $\uparrow$   
                     & LPIPS $\downarrow$  & PSNR $\uparrow$ & SSIM $\uparrow$   \\ 
                \midrule
                \midrule
                GaussianAvatars &   0.2257   &  17.11 &  82.09   & 0.2137   &  17.50  &  83.05 \\
                \midrule
                no condition-6k        
                    &  0.2361   &  14.37  &  84.84    &  0.2147  &  15.37  & 86.14  \\
                landmark condition -5k  
                    &  0.2095    & 18.40  &  87.66   & 0.1984  & 18.58  & 88.24  \\
                \midrule
                 %w/o personalized, $\set{L}_{SDS}$         
                 %   &  0.2543    & 14.43  & 82.76    & 0.2082  &  17.01 & 83.85  \\
                 w/o personalization, $\set{L}_{RGB}$ -5k   
                    &  0.1868    & 17.16  &  85.66  & 0.1745  &  17.83 &  86.49 \\
                personalized,  $\set{L}_{SDS}$              
                    &  0.1918    &  17.07  & 86.97    &  0.1863    &  17.29  &  87.44 \\
                single-stage personalization, $\set{L}_{RGB}$6k 
                    & 0.1784   &  17.15 &  87.57   &  0.1681 &  17.67 &  88.21 \\
                \midrule
               % w/o $\set{L}_{expr}$ 
               %     &  \bf 0.1605   &  \bf 17.68  &  87.84  & \bf  0.1503 & \bf 18.17  & 88.42  \\
                Ours  
                    & 0.1690   &  17.58  &  \bf 88.02  & 0.1581 & 18.06   &  \bf 88.84  \\
                \bottomrule
        \end{tabular}
        \vspace{5mm}
        \caption{Ablation Studies on the 'EMO-1' sequence of subject $\#$306 in the Nersemble~\cite{} dataset. } 
        \label{tab:ablation}
        \end{center}
\end{table}

==> tex_cvpr/additional_figure.tex <==
%
\begin{figure*}[t]
    %\vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth]{figs/compare_novelview.pdf}
    \begin{tabular*}
        {\linewidth}{
            @{\extracolsep{\fill}}
            p{0.13\linewidth}
            p{0.11\linewidth}
            p{0.13\linewidth}
            p{0.15\linewidth}
            p{0.10\linewidth}
            p{0.16\linewidth}
        }
        \centering (a) Input frame
        & \centering (b) INSTA
        & \centering (c) FlashAvatar
        & \centering (d) GaussianAvatars
        & \centering (e) Ours
        & \centering (f) Ground truths\\
    \end{tabular*}
    \vspace{-4mm}
    \caption{\textbf{Novel view synthesis from monocular videos on the Nersemble dataset.} Compared to state-of-the-art methods, our method consistently produces more favorable renderings from both near and far hold-out views, and captures more accurate facial expression details.}
    \label{fig:novelview}    
\end{figure*}
%
\begin{figure*}[h]
    \centering
    \includegraphics[width=.9\linewidth]{figs/novelview_real.jpg}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}p{0.07\linewidth}p{0.12\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.10\linewidth}p{0.20\linewidth}}
    \centering & (a) Input frame & \centering (b) INSTA & \centering (c) FlashAvatar & \centering (d) GaussianAvatars & \centering (e) Ours & \\
    \end{tabular*}
    \caption{\textbf{Novel view synthesis on in-the-wild monocular videos.} Given a sequence captured from the front view, our approach can still generate photo-realistic novel-view renderings, even from an extreme side view (bottom). However, existing methods fail to extrapolate to this case.}
    \label{fig:novelview_real}
\end{figure*}

%
\begin{figure*}[!htp]
    \centering
    \includegraphics[width=\linewidth]{figs/compare_reenact.pdf}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
    \centering (a) Driving frame & \centering (b) Source Identity & \centering (c) INSTA & \centering (d) FlashAvatar & \centering (e) GaussianAvatars & \centering (f) Ours \\
    \end{tabular*}
    \vspace{-6mm}
    \caption{\textbf{Self Reenactments from Monocular videos on the Nersemble dataset.}
    We use the tracked FLAME pose and expressions of a driving sequence to animate the reconstructed Gaussians.
    Our method demonstrates better generalization ability to novel expressions and produces higher quality novel views.
    }
    \label{fig:selfnact}
\end{figure*}
%
\begin{figure*}[!htp]
    \centering
    \includegraphics[width=\linewidth]{figs/compare_reenactcross.pdf}
    \begin{tabular*}
        {\linewidth}{@{\extracolsep{\fill}}p{0.15\linewidth}p{0.16\linewidth}p{0.13\linewidth}p{0.16\linewidth}p{0.14\linewidth}p{0.16\linewidth}p{0.09\linewidth}}
        \centering (a) Driving frame & \centering (b) Source Identity & \centering (c) INSTA & \centering (d) FlashAvatar & \centering (e) GaussianAvatars & \centering (f) Ours \\
    \end{tabular*}
    \vspace{-6mm}
    \caption{\textbf{Cross-Reenactments from Monocular videos on the Nersemble dataset.} 
    Our method outperforms state-of-the-art methods by showcasing more vivid expression transfers and more plausible renderings around the mouth region.}
    \label{fig:crossnact}
\end{figure*}


